VLMbench: A Compositional Benchmark for Vision-and-Language Manipulation

Benefiting from language flexibility and compositionality, humans naturally intend to use language to command an embodied agent for complex tasks such as navigation and object manipulation. In this work, we aim to fill the blank of the last mile of embodied agents -- object manipulation by following human guidance, e.g., "move the red mug next to the box while keeping it upright." To this end, we introduce an Automatic Manipulation Solver (AMSolver) system and build a Vision-and-Language Manipulation benchmark (VLMbench) based on it, containing various language instructions on categorized robotic manipulation tasks. Specifically, modular rule-based task templates are created to automatically generate robot demonstrations with language instructions, consisting of diverse object shapes and appearances, action types, and motion constraints. We also develop a keypoint-based model 6D-CLIPort to deal with multi-view observations and language input and output a sequence of 6 degrees of freedom (DoF) actions. We hope the new simulator and benchmark will facilitate future research on language-guided robotic manipulation.

==> 3_simulator.tex <==
\begin{figure}[!tbp]
% \flushright
\includegraphics[width=\columnwidth]{images/unit_task.pdf}
\vspace{-4ex}
\caption{The unit task templates in the AMSolver. On the left, we show three main common task types of household tasks and give several example tasks for each. On the right, we show three unit task templates parameterized by position and orientation constraints over the robot end-effector on either goal pose or entire path. By combining these unit task templates, various task examples can be generated.}
\label{fig:unit_task}
\end{figure}

We consider three main categories of household manipulation tasks: rearrangement (move an object from place to place, e.g., collect trash into the bin), affordance usage (exploit particular usage of some object, e.g., pour water from a mug), and multi-step tasks (can be decomposed into several individual steps, e.g., connect every two pieces to assemble a table from parts). To formulate a unified task representation, we assume that every task within these categories can be considered a combination of objects and unit actions. To describe the essential elements of tasks, we proposed Automatic Manipulation Solver (AMSolver)\footnote{AMSolver is implemented in CoppeliaSim~\cite{6696520} (Free Educational License)~\url{https://www.coppeliarobotics.com/} and codes are based on RLbench~\cite{james2020rlbench}(RLBench Software License)~\url{https://github.com/stepjam/RLBench} and PyRep~\cite{james2019pyrep}(MIT License)\url{https://github.com/stepjam/PyRep}.}, a rule-based automatic task builder consisting of object-centric representations and unit task templates, as shown in Fig.~\ref{fig:unit_task}. Below we illustrate how a complex task can be built bottom-up.
% We explain how complex tasks can be built based on the proposed concepts in the following paragraphs.

\subsection{Rule-based Unit Tasks}

Since the tasks have notable variations, we assume that each complex task can be decomposed into the combinations of several unit tasks from the aspects of end-effector trajectories. We define a \textit{unit task} as the semantic step of completing a sub-goal of the entire task. 
% A \textit{unit task} should keep an invariant rule among different tasks, consisting of a simple structure, and have enough scalability to represent every task step. 
Specifically, a unit task is defined in a formula of `take action on an object under certain constraints' where a unit task can be parameterized by two constraints: (a) \textbf{position constraints} and (b) \textbf{orientation constraints}, which describe the valid spatial space or orientation range, respectively, of the end-effector for a specific task.
We propose three unit task templates detailed below that can compose the aforementioned complex tasks.
\\
\noindent\textbf{Control} is a preparation or ending step of a task, which models the transition of the object state, where the state indicates whether the robot can move the object or not. In this work, we specify one way of transition: to obtain control by grasping it and release control by opening the gripper. There are other ways to obtain control, like pushing, hitting, etc. However, these transitions will naturally lead to the constraints in the following sub-tasks, so they cannot be considered a general component for any complex task.
% Due to the generalization, we only consider grasping in this work. 
In this unit task, the position and orientation constraints depend on the geometry of object instances. 
% a robot either can \textbf{a1} grasp objects, or get in contact with objects to begin to \textbf{a2} push; to release control, the robot can \textbf{a3} release objects from grasping or detach contact with objects from pushing. For these two basic actions, we assume every object used in the task is \textit{pushable} (so it's not mentioned in object property), while only some objects are \textit{graspable}. Examples of this unit task include \textbf{T0(a1,b1)}: grasping a graspable object, and \textbf{T0(a2,b2)}: beginning to push an object that is not graspable.
\\
\noindent\textbf{M1} denotes moving the target object with goal pose constraints (position and orientation constraints), which can be modeled as a 6 DoF transform in the robot's workspace. The position constraints define a bounded goal space in $\mathbb{R}^3$, while the orientation constraints define a valid 3D orientation $SO(3)$. We consider four types of position constraints: (a1) \textit{Free}, (a2) \textit{Plane}, (a3) \textit{Line}, and (a4) \textit{Fixed}, which means the goal position is any point inside a 3D space (a1), constrained in a 2D plane (a2), constrained in a line-shape area (a3), or fixed to a certain point (a4). There are three types of orientation constraints: (b1) \textit{Free}, (b2) \textit{Axis}, and (b3) \textit{Fixed}, which means the goal orientation is unlimited in 3D rotation space (b1), only rotated along an axis in space (b2), or fixed at a given orientation (b3). For example, M1[a2, b1] can represent placing the object on a tabletop (with plane position constraint), while M1[a3, b2] can represent moving the object to a position on one line and ending with a constrained orientation of one axis, like dropping a stick into the hole.
\\
\noindent\textbf{M2} denotes moving the target object along a trajectory while satisfying the motion constraints during the entire path, which implies a more strict condition than \textbf{M1}. The constraints are mostly from object articulation or task-specific requirements. If the target object has a joint that only supports rotation or sliding motion, the robot path should naturally obey these physic designs, reflecting on position and orientation constraints. On the other hand, a hingeless object will be restrained by the goal of the task. Therefore, there are four kinds of position constraints: (a1) \textit{Free}, (a2) \textit{Plane}, (a3) \textit{Line}, and (a4) \textit{Fixed trajectory}, which means any position inside a space (a1), a plane (a2), a line (a3) or a predefined path (a4) should be feasible for the trajectory, and four kinds of orientation constraints: (b1) \textit{Free}, (b2) \textit{Axis}, (b3) \textit{Fixed}, and (b4) \textit{Depend on position}, which means every pose in the trajectory should be unlimited orientations (b1), at most rotated along an axis (b2), fixed to a certain orientation (b3), or depended on the corresponding positions. For example, M2[a2, b2] means moving the object inside a 2D plane with maintaining the orientation of one axis, like wiping the table, while M2[a4, c2] means moving the object along a fixed trajectory with maintaining the orientation of one axis, like using a screwdriver to tighten a screw. It is worth mentioning that M2[a1,b1] will degenerate to M1[a1,b1].

According to our unit task definition, we have covered every feasible 6 DoF poses of the end-effector. Therefore, we have reason to believe that these unit tasks can represent any complex task in the action space.

\subsection{Object-centric Representation}
Some recent works~\cite{li2021igibson,yuan2022sornet} have used object-centric representations for manipulation. Since the properties are defined on objects, these representations can easily cross the variations of environments, agents, and tasks. Our benchmark assumes that objects used in the tasks are rigid, and their fundamental properties will not change during the tasks. Therefore, we can parameterize the objects as a set of configurations, including class, color, size, and geometry shape. If the object is articulated, its whole configuration will contain the configuration of each part and the physical constraint of each connection. For example, a door consists of three parts: the door base, plank, and handle, so its configuration will contain each part's configuration and record the positions and ranges of two revolute joints. 

Since grasping is a prerequisite for many tasks, we create an object-wise grasp pose dictionary. Specifically, a point cloud-based grasping pose detection algorithm~\cite{ten2017grasp} is implemented to search all feasible grasping poses automatically, given the object's shape and robot gripper parameters. The grasp poses are saved in the object's local coordinate frames and can then be transformed to world space for a particular task by simply multiplying with the object's pose.

\subsection{Task Creation}
To generate demonstrations for semantic tasks, we need to use the predefined unit task sequence combined with object configurations and goal conditions. The goal conditions are the feasible goal pose sets of the current manipulated object for each unit task. The goal conditions can be formatted as bounding boxes, planes, lines, joint angles, or generated by functions for special pose sets. For example, a rearrangement task \textit{``Put the ball into the basket"} needs to transit a ball into the empty space of the basket without any constraints requirement, which means the goal condition of the ball is a set of poses inside the blank space of basket. Then, we can format this task as $(Control, ball) + (M1[a1, b1], ball)$. Note that \textit{ball} can be replaced with other objects, so $(Control, object)+ (M1[a1, b1], object)$ can represent any pick-and-place task without specific constraints. 
Another example is \textit{``Pour the water from one mug to another"}. This task needs to keep the mug opening upward during the move towards the top of another mug. We can format this task as $(Control, source\ mug) + (M2[a1, b2], source\ mug) + (M2[a4, b4], source\ mug)$. For the first $(M2[a1, b2], source\ mug)$, the goal condition should make the horizontal distance between the geometry centers of two mugs less than the half-height of the source mug, and the vertical distance should be larger than the height of the container mug. Therefore, the goal condition is a set of poses, calculated by a function using the geometry and poses of two mugs.

Overall, the unit task sequence can be unlimitedly superposed to create any length of multi-step tasks. Once the sequence and goal conditions are defined, if there are valid trajectories to finish the task, our AMSolver will automatically generate a demonstration trajectory to solve the task.

% \subsection{Implementation Details}
% The AMSolver is built inside the CoppeliaSim~\cite{6696520} environment and written in Python and Lua based on RLbench~\cite{james2020rlbench} and PyRep~\cite{james2019pyrep}. The agent is a Franka Emika Panda robot arm with 7 DoF, standing on a wooden table. To achieve the grasping ability for any object shape, we implement one version of the algorithm of ten Pas et al.~\cite{ten2017grasp}. The generator will calculate the normals and principal axis of partial point clouds. Then, the normals, principal axis, and cross-product will establish the grasp poses. Finally, the agent will calculate inverse kinematic to check the validation. More details can be found in~\cite{ten2017grasp}. Each unit task will generate one waypoint as the sub-goal of the end-effector or one fixed cartesian path as the fixed sub-trajectory for the end-effector in the environment. We use the OMPL library~\cite{sucan2012the-open-motion-planning-library} to find a valid trajectory between two waypoint configurations. In the end, we will get a valid path from the beginning to the task finish, consisting of the critical waypoints information.

==> 6_experiment.tex <==

\subsection{Experimental Setup}
Before testing each baseline, we preprocess the tasks to help the agent eliminate trivial steps. 1) We divided tasks into the sub-goal sequences by the ground truth waypoints generated by AMSolver, so that the agent only needs to estimate the actions of the predefined unit task sequence for each task. 2) Since we have the ground truth gripper state for each sub-goal, we also provide whether the gripper should open or close for each action estimation. 3) To increase the grasping stability, we use the ground truth grasping pose instead of estimations if these two poses are close enough (distance is less than 5 cm and the rotation is less than 10 degrees). 4) To reduce the fail grasping cases due to the motion planning, we use a predefined pre-grasping offset, which is 8cm backward along the z-axis of the target grasping pose, and a post-grasping offset, which is 8cm upward along the z-axis of the world frame.

\begin{table}[tbp]
\caption{The task success rates of different agents in each task category. For Unimodal agents in the table fail in almost tasks expect the success of Image-Language agent on the ``Pick \& Place" tasks. 6D-CLIPort (GT Ori) and 6D-CLIPort (GT Pos) denote the 6D-CLIPort with ground truth orientations or positions for the ablation study.}
\label{table:tasks_result}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrr}
\toprule
\textbf{Agent}               & \textbf{Pick} \& \textbf{Place} & \textbf{Stack} & \textbf{Drop}  & \textbf{Shape Sorter} & \textbf{Pour} & \textbf{Wiper} & \textbf{Drawer} & \textbf{Door}  \\ \midrule
Unimodal            & 3.61          & 0.00  & 0.00  & 0.00         & 0.00 & 0.00  & 0.00   & 0.00  \\
6D-CLIPort          & 20.83         & 7.66  & 5.23  & 14.47        & 1.05 & 6.96  & 16.67  & 18.75 \\ \midrule
6D-CLIPort (GT Ori) & 26.94         & 11.91 & 18.02 & 14.89        & 1.58 & 6.25  & 26.67  & 27.50 \\
6D-CLIPort (GT Pos) & 85.56         & 62.13 & 18.60 & 62.13        & 0.00 & 74.22 & 36.67  & 28.75 \\ \bottomrule
\end{tabular}%
}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[tbp]
\centering
\caption{Task success rate of different properties across task categories.}
\label{table:vars_result}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrr}
\toprule
\textbf{Agent} & \textbf{Color} & \textbf{Shape} & \textbf{Size} & \begin{tabular}[c]{@{}c@{}}\textbf{Relative}\\ \textbf{Position}\end{tabular} & \textbf{Direction} & \textbf{Level} & \textbf{Action Type} & \textbf{Amount} \\ \midrule
Unimodal            & 0.40  & 2.00  & 0.95  & 1.47  & 0.00  & 0.00  & 0.00  & 0.00  \\
6D-CLIPort          & 9.07  & 19.00 & 9.52  & 11.76 & 10.00 & 16.67 & 17.86 & 17.86 \\ \midrule
6D-CLIPort (GT Ori) & 13.89 & 14.41 & 18.00 & 19.05 & 6.67  & 26.67 & 27.14 & 27.14 \\
6D-CLIPort (GT Pos) & 52.59 & 52.65 & 72.50 & 45.24 & 80.00 & 36.67 & 32.14 & 32.14 \\ \bottomrule
\end{tabular}%
}
\end{table}

\subsection{Baselines}
In order to test the influence of different modalities, we also trained on other four unimodal agents: \textit{Image-Language}, \textit{Depth-Language}, \textit{Blind-Language}, and \textit{Image-Depth}. These agents use the same attention mechanism as 6D-CLIPort but have different structures in the encoding module. To clarify, the Image-Language agent uses the CLIP for RGB and language in each module. The Depth-Language agent uses the Transporter ResNet~\cite{zeng2020transporter} for depth image and a pretrained DistilBERT~\cite{sanh2019distilbert} to extract language features. The Blind-Language agent will only use a pretrained DistilBERT for feature map estimation. And Image-Depth agent has the same structure as the Depth-Language agent, but the language will only include the prompt for steps indication without high-level language instructions.

\subsection{Results}
The results of baseline agents are shown in Table~\ref{table:tasks_result}. We find out that the unimodal models perform poorly in every task. Except for the Image-Language agent achieving a 3.61\% success rate on the pick and place tasks, other agents, including the Depth-Language agent, Image-Depth agent, and Blind-Language agent, fail in all tasks. The results of the Image-Language agent show the importance of RGB and language in our benchmark. Compared to the results of the 6D-CLIPort agent, the feature fusion of RGB, depth, and language can significantly improve the performance. Compared with the different results of 6D-CLIPort on each task category, we can find that the agent has better performance on the ``Plick \& Place", ``Shape Sorter," ``Drawer," and ``Door" tasks. The trajectories of these tasks have fewer variations than others. It shows that the 6D-CLIPort can successfully finish the tasks in 6 DoF spaces. The common characteristic of other tasks is the requirement of high precision 6 DoF actions or the need to keep constraints during the tasks, where the 6D-CLIPort agent lacks such ability. We also show the results of the agents on each task variation in Table~\ref{table:vars_result}. The results indicate that the 6D-CLIPort agent is sensitive to variations of shape, amount, and action type, which show the reasoning ability of the agent in both object and action spaces.

\subsection{Ablations Study}
In order to measure the learning ability of 6D-CLIPort, we individually test the position estimations and orientation estimations by giving the ground truth values of the waypoint. Although the trajectories of finishing the tasks are various, and we cannot obtain the optimal position and rotation by partly giving orientation and position estimations, we can regard the poses of waypoints as sub-optimal solutions. 6D-CLIPort (GT Ori) denotes the 6D-CLIPort with the orientations of waypoints. 6D-CLIPort (GT Pos) denotes the 6D-CLIPort with the positions of waypoints. The results are shown in Table.~\ref{table:tasks_result} and Table.~\ref{table:vars_result}. From the results, we can find out that the position estimations limit the performance of 6D-CLIPort in ``Pick \& Place", ``Stack" and ``Shape Sorter" tasks. For the tasks that needed high precision rotations, e.g. ``Drop," and ``Pour," the 6D-CLIPort cannot predict robust orientations, which prove the conclusion above.

%Since the CLIPort only can estimate three degrees of freedom, we provide other degrees with ground truth values, including the height $z$, the rotation along the x-axis $r_x$, and the rotation along the y-axis $r_y$. Although the ground truth waypoints in the trajectories are highly related to each others, their values can be considered as a sub-optimal solution for the estimations of CLIPort. On the one hand, compared to the results from action spaces, we can find that both agents perform well on 'pick and place' and 'wipe the table' tasks. These two tasks either do not need the high precision of the height and rotations or only have subtle variations on the height and rotations along the x-axis and y-axis. And they both perform badly on the "pour water" tasks since this task needs high precision action pose and the next step should be highly related to the previous step. Then, we find both agents have poor performance on the other tasks but 6D-CLIPort worse. The common characteristic of these tasks is the requirement of high precision 6 DoF actions. There is still huge progress space for these action estimations. On the other hand, the agent have different performances on each variations.


==> checklist.tex <==

\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Please see Abstract and Section~\ref{sec:intro}}
 \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Please see Section~\ref{sec:discussion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Please see Section~\ref{sec:discussion}}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Please see it in Appendix. We present the implementation details there.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please see it in Appendix}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Please see it in Appendix}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please see it in Appendix}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Please see Section~\ref{sec:amsolver} and ~\ref{sec:agent}}
  \item Did you mention the license of the assets?
    \answerYes{Please see Section~\ref{sec:amsolver} and ~\ref{sec:agent}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Please see it in Appendix}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We follow the open-source agreement and its license strictly.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{The dataset has no sensitive or personally identifiable information.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

